TIMBRE: Efficient Job Recommendation On Heterogeneous Graphs For Professional Recruiters

Job recommendation gathers many challenges well-known in recommender systems. First, it suffers from the cold start problem, with the user (the candidate) and the item (the job) having a very limited lifespan. It makes the learning of good user and item representations hard. Second, the temporal aspect is crucial: We cannot recommend an item in the future or too much in the past. Therefore, using solely collaborative filtering barely works. Finally, it is essential to integrate information about the users and the items, as we cannot rely only on previous interactions. This paper proposes a temporal graph-based method for job recommendation: TIMBRE (Temporal Integrated Model for Better REcommendations). TIMBRE integrates user and item information into a heterogeneous graph. This graph is adapted to allow efficient temporal recommendation and evaluation, which is later done using a graph neural network. Finally, we evaluate our approach with recommender system metrics, rarely computed on graph-based recommender systems.

==> sections/background.tex <==
\section{Background }

In this paper, we are going to consider heterogeneous graphs. A heterogeneous graph $G$ is defined by a tuple $(V, R, T, E, \Omega)$ where V is a finite set of nodes, $R$ is a finite set of relationships, $T$ is a set of types, $E \subset V \times R \times V$ is the set of edges, and $\Omega \subset E \times T$ is the set of types associated to a node. We can associate properties with the nodes or edges of a heterogeneous graph using a function $P(v_1)$ or $P(v_1, r, v_2)$ where $v_1 \in V$, $v_2 \in V$, and $r \in R$. When the property represents temporal information, we talk about a temporal heterogeneous graph. In general, this information represents the date of creation of a node or edge.


==> sections/baselines_long.tex <==
\paragraph{Baselines}

We compared our approach with the following state-of-the-art approaches:
\begin{itemize}
    \item Temporal Graph Network~\cite{rossi2020tgn}, or TGN, is a standard inductive framework based on continuous-time dynamic graphs if required.
    \item Neighbour Aware Temporal Network~\cite{luo2022nat}, or NAT, is a method that replaces the traditional single-vector representation with a dictionary-type representation. By storing the key of a neighbor node in the dictionary, they essentially get a more precise representation of the structural context of a given set of nodes. They also store each updated representation of the nodes in a dedicated data structure called N-cache.
    \item JODIE~\cite{kumar2019jodie} trains a Recurrent Neural Network (RNN) to learn the embedding trajectories of users and items. This allows for an update of the embedding of both user and item nodes at each interaction. The RNN is also employed to predict future representation and, thus, future user-item interaction.
    % \item TGAN~\cite{xu2021tgan} aggregate temporal features of neighbor nodes through a graph attention layer.
    \item DYREP~\cite{trivedi2018dyrep} models the change of the representation of the node by taking into account the dynamic of the graph (the structure of the graph might change) and the dynamic on the graph (the nature of the communication between the node might change). To do so, it uses a temporal attention mechanism which learns to focus on the appropriate neighbors.
    \item TGSRec~\cite{fan2021continuous} is a graph recommender system based on attention. It models both the collaborative signals from the users and items, and the temporal dynamics. We reused the code provided by the authors but modified the evaluation setup. The original paper removed all the users who were not in the train set from the validation and test sets. It makes the task much easier as the cold start problem disappears, and it drastically reduces the size of the validation and test set as the split was done before the removal (the higher the time gap between a data point and the train set, the less likely the user and the item are to be in the train set).
\end{itemize}

==> sections/limitations_future_work.tex <==
\section{Limitations and Future Work}

In this paper, we discuss job recommendations, an area often prone to discrimination. We did our best to remove any feature related to gender or ethnicity.

As our ablation study shows, including features in the graph is not necessarily trivial and might require further consideration. For example, although the company itself is not relevant, the company's sector may be interesting. That would allow the inclusion of previous positions in the graph. For the sparse features, it might be worth finding a way to find them. However, it would require significant human labor. A possible future work would be to have a human-in-the-loop system in which we suggest candidates and ask for further information.
